A Model Parallel Proximal Stochastic Gradient Algorithm for Partially Asynchronous Systems

Large models are prevalent in modern machine learning scenarios, including deep learning, recommender systems, etc., which can have millions or even billions of parameters. Parallel algorithms have become an essential solution technique to many large-scale machine learning jobs. In this paper, we propose a model parallel proximal stochastic gradient algorithm, AsyB-ProxSGD, to deal with large models using model parallel blockwise updates while in the meantime handling a large amount of training data using proximal stochastic gradient descent (ProxSGD). In our algorithm, worker nodes communicate with the parameter servers asynchronously, and each worker performs proximal stochastic gradient for only one block of model parameters during each iteration. Our proposed algorithm generalizes ProxSGD to the asynchronous and model parallel setting. We prove that AsyB-ProxSGD achieves a convergence rate of $O(1/\sqrt{K})$ to stationary points for nonconvex problems under \emph{constant} minibatch sizes, where $K$ is the total number of block updates. This rate matches the best-known rates of convergence for a wide range of gradient-like algorithms. Furthermore, we show that when the number of workers is bounded by $O(K^{1/4})$, we can expect AsyB-ProxSGD to achieve linear speedup as the number of workers increases. We implement the proposed algorithm on MXNet and demonstrate its convergence behavior and near-linear speedup on a real-world dataset involving both a large model size and large amounts of data.

==> src/asyn_bspg.tex <==
%!TEX root = ../main.tex

\section{Asynchronous Block Stochastic Proximal Gradient Descent}
\label{sec:baspg}

In this section, we consider a block-wise extension of Algorithm~\ref{alg:apsgd-global} into an algorithm that we call B-AsynSPG. The role of workers is the same as is in Algorithm~\ref{alg:apsgd-global}, except that each worker only updates one block of $x$ per iteration. Since updating a block does not require locking all the model parameters, this is also called a \emph{lock-free} algorithm in the literature, and can be implemented in shared memory systems, e.g., multi-core and multi-GPU systems. 
%Following the seminal work of HOGWILD!\cite{recht2011hogwild}, many studies have demonstrated that near linear speedups are achievable on several machine learning tasks via asynchronous, lock-free implementations, e.g., \cite{liu2015asynchronous}. In all of these studies, classic algorithms are parallelized by simply running parallel and asynchronous model updates without locks. These lock-free, asynchronous algorithms exhibit speedups even when applied to large, non-convex problems, as demonstrated by deep learning systems such as Google’s Downpour SGD \cite{dean2012large}, Microsoft’s Project Adam \cite{chilimbi2014project} and Parameter Server \cite{li2014scaling}.

Our block-wise asynchronous parallel SPG algorithm is described in Algorithm~\ref{alg:abpsgd-global}. 
Assume the model $x$ can be divided into $M$ blocks, each stored on a separate parameter server.
There are a few characteristics of this algorithm. The procedure for each worker is similar as is in Algorithm~1. 
 \emph{First}, in each iteration, each worker atomically updates one block of $x$ instead of the entire $x$.
\emph{Second}, when each worker reads model parameters $x$ from the servers, different blocks of $x$ may experience different degrees of delays. This is because in a blockwise algorithm, the writes to different blocks can be made by different workers and at different times. The inconsistent model parameters are a key difference of Algorithm~\ref{alg:abpsgd-global} from Algorithm~\ref{alg:apsgd-global}. \emph{Finally}, each worker must take $N$ random samples from its own local dataset and computes the averaged stochastic gradient of these samples, i.e.,
%\emph{Firstly}, the iterates are allowed to be inconsistent so we do not need any software lock. When a processor tries to update $x$ even other processors are reading $x$ in the time. \emph{Secondly}, all updates are performed on one single block $x_j$ at each time slot. Therefore, parallelism on $x$ is met, which reduces the likelihood of IO conflict. \emph{Thirdly}, in each iteration, multiple samples are drawn and gradients are calculated in parallel, like Algorithm~\ref{alg:apsgd-global}. 
when a worker pushes a stochastic gradient to a server, it is the averaged gradient of $N$ samples (although the gradients of different samples even in a same batch are allowed to be calculated using different ``dirty'' versions of $x$), i.e.,
{\small
\begin{equation}
	\hat{G}_{j_k}^{k} := \frac{1}{N}\sum_{i=1}^N \nabla_j F(\hat{x}^{k,i}; \xi_{k, i}),
	\label{eq:grad_abspg}
\end{equation}
}
% which is an extension from \eqref{eq:grad_aspg} by replacing $x$ to $\hat{x}$ since each node cannot obtain a vector from inconsistent read. This also implies that, the parallelism on training data is also met. Therefore, the proposed AsynBPSG algorithm is with \emph{data parallelism} and \emph{model parallelism}.
where $\hat{x}$ is a ``dirty'' version of $x$ due to inconsistency.  
% We now put more elaborations on \emph{inconsistent read} for shared memory systems. At iteration $k$, we have
To precisely characterize this implementation and especially represent $\hat{x}$, we monitor the value of  $x$ in the shared memory. We define one iteration as a modification on any single block of $x$ in the shared memory; the update of each single block is considered to be atomic. We use $x^k$ to denote the value of $x$ in the shared memory after $k$ iterations of the algorithm and $\hat{x}^{k,i}$ to denote the ``dirty'' copy of $x$ read from the shared memory when used for computing the gradient of sample $\xi_{k, i}$ at the $k$-th iteration. %$\hat{x}^k$ can be represented by $x^k$ with a few earlier updates missing
We have
{\small
\begin{equation}
	\hat{x}^{k,i} = x^k + \sum_{l \in K(\bm{\tau}(k, i))} x^{l} - x^{l+1},
\end{equation}
}
where $\bm{\tau}(k, i)=(\tau_1(k,i), \tau_2(k,i),\ldots, \tau_M(k,i))$ denotes the \emph{delay vector}, i.e., the delays of different blocks in $\hat{x}^{k,i}$ when computing the gradient for sample $\xi_{k, i}$ at iteration $k$, where $\tau_j(k, i)$ is the delay of a specific block $x_j$. Given a vector $\bm{\tau}(k, i)$, the \emph{delay set} $K(\bm{\tau}(k, i))$ is defined as the set of non-zero delay values in $\bm{\tau}(k, i)$\footnote{For example, suppose $\bm{\tau}(k, i)=(0,1,3)$, then we have set $K(\bm{\tau}(k, i)) = \{1, 3\}$.}, which will be used in our analysis.
% When we have $N$ samples as a mini-batch, we denote $\bm{\tau}(k, i)$ as the delay vector when computing gradient w.r.t sample $\xi_{k,i}$, and $K(\bm{\tau}(k, i))$ as its corresponding delay set.
% that consists of iterations in $\bm{\tau}(k)$ 
% To reflect the delay for all samples $\xi_{k,1},\ldots, \xi_{k,M}$, we also use $\bm{\tau}(k, i)$ and $K(\bm{\tau}(k, i))$ to denote the block delay distribution vector and the delay set, respectively, for participant $i$ at iteration $k$.

\setlength{\intextsep}{0pt}
\begin{wrapfigure}{l}{0.5\textwidth}
\begin{minipage}{0.5\textwidth}
\begin{algorithm}[H]
\caption{B-AsynSPG (a Global Perspective)}
\label{alg:abpsgd-global}
\begin{algorithmic}[1]
\State Initialize $x_1$.
\For {$k=1,\ldots, K$}
\State {Randomly select $N$ training samples indexed by $\xi_{k, 1}, \ldots, \xi_{k, N}$.}
\State {Randomly select an index $j_k$ from $\{1,\ldots, M\}$ }.
\State {Calculate the averaged gradient $\hat{G}_{j_k}^k$ according to \eqref{eq:grad_abspg}.}
\State {$x_{j_k}^{k+1} \gets \prox{\eta_k h_{j_k}}(x_{j_k}^{k} - \eta_k \hat{G}_{j_k}^{k})$.}
\EndFor
\end{algorithmic}
\end{algorithm}
\end{minipage}
\end{wrapfigure}
\setlength{\intextsep}{0pt}

\subsection{Convergence Analysis}
To analyze Algorithm~\ref{alg:abpsgd-global}, we make the following common assumptions \cite{recht2011hogwild,liu2015asynchronous,avron2015revisiting}:
\begin{assumption}[Bounded delay]
	All entries in $\bm{\tau}(k, i)$ should be upper bounded by $T$. That is, for all $k$ and $i$, we have $\min K(\bm{\tau}(k, i)) \geq k-T$. Also, the number of elements in $K(\bm{\tau}(k, i))$ is at most $T$: $|K(\bm{\tau}(k, i))| \leq T$.
	\label{asmp:bound2}
\end{assumption}
\begin{assumption}[Independence]
	All random variables including selected indices $\{j_k\}$ and $\{\xi_{k, i}\}$ for all $k$ and $i$ in Algorithm~\ref{alg:abpsgd-global} are mutually independent. 
	\label{asmp:indie2}
\end{assumption}
% In the inconsistent read mode, each block has its own delay and therefore the maximum delay should be bounded per block. Here $T$ is similar with that in Assumption~\ref{asmp:bound1} and is roughly proportional to the number of workers as well. 
With inconsistent reads/writes, we assume that both the maximum delay per block and the number of delayed blocks should be bounded by $T$, which is roughly proportional to the number of workers. This is similar to the bound in Assumption~\ref{asmp:bound1}.
The independence assumption is also widely used for convergence analysis. We also need Assumptions \ref{asmp:smooth}, \ref{asmp:unbias_grad} and \ref{asmp:var_grad} here. %Note that the gradient is calculated on the entire $x$. Thus, we cannot make a block-wise Lipschitz assumption on gradients. Fortunately, this is not a big issue when choosing a block to be updated in a uniformly random fashion.

The following theorem is our main result for B-AsynSPG convergence analysis:
\begin{theorem}
	% If Assumptions~\ref{asmp:bound2} and \ref{asmp:indie2} hold,  and t
	If the step length sequence $\{\eta_k\}$ in Algorithm~\ref{alg:abpsgd-global} satisfies
	{\small
	\begin{equation}
		\eta_k \leq \frac{1}{16L_{\max}},\quad 6\eta_k L^2 T \sum_{l=1}^T \eta_{k+l} \leq M^2,
	\end{equation}
	}
	for all $k=1,2,\ldots, K$, we have the following ergodic convergence rate for Algorithm ~\ref{alg:abpsgd-global}:
	{\small
	\begin{equation}
	\begin{split}
&\quad\ \frac{\sum_{k=1}^K (\eta_k - 8L_{\max}\eta_k^2) \norm{P(x^k, g^k, \eta_k)}^2}{\sum_{k=1}^K \eta_k - 8L_{\max}\eta_k^2} \\
& \leq \frac{8M(\Psi(x^1) - \Psi(x^*))}{\sum_{k=1}^K \eta_k - 8L_{\max}\eta_k^2} + \frac{8M \sum_{k=1}^K \left( \frac{L\eta_k^2}{MN} + \frac{3\eta_kL^2 T\sum_{l=1}^T \eta_{k-l}^2}{2M^3 N} \right) \sigma^2}{\sum_{k=1}^K \eta_k - 8L_{\max}\eta_k^2},
	\end{split}
	\end{equation}
	}
	where the expectation is taken in terms of all the random variables in Algorithm~\ref{alg:abpsgd-global}.
	\label{thm:abspg_convergence}
\end{theorem}

Taking a closer look at Theorem~\ref{thm:abspg_convergence}, we can properly choose the learning rate $\eta_k$ as a constant value and obtain the following results on convergence rate:
\begin{corollary}
	% Assume that Assumptions \ref{asmp:smooth}, \ref{asmp:unbias_grad} and \ref{asmp:var_grad} hold. 
	Let the step length be a constant, i.e., 
	{\small
	\begin{equation}
	    \eta := \sqrt{\frac{(\Psi(x_1) - \Psi(x^*))M N}{LK\sigma^2}}.
	\end{equation}
	}
	If the delay bound $T$ satisfies
	{\small
	\begin{equation}
	    K \geq \frac{128(\Psi(x_1) - \Psi(x_*)) N L}{M^3 \sigma^2} (T+1)^4,
	\end{equation}
	}
	then the output of Algorithm~\ref{alg:abpsgd-global} satisfies the following ergodic convergence rate as
	{\small
	\begin{equation}
	% \begin{split}
		\mathop{\min}_{k=1,\ldots,K} \mathbb{E}[\norm{P(x_k, g_k, \eta_k)}^2] \leq \frac{1}{K}\sum_{k=1}^K \mathbb{E}[\norm{P(x_k, g_k, \eta_k)}^2] \leq 32\sqrt{\frac{2(\Psi(x_1) - \Psi(x_*))LM\sigma^2}{KN}}.
	% \end{split}
	\end{equation}
	}
	% \vspace{-3mm}
	\label{corr:abspg_convergence}
\end{corollary}

We now make a few remarks for this corollary. We first compare results between Corollary~\ref{corr:aspg_convergence} and Corollary~\ref{corr:abspg_convergence}. Like Corollary~\ref{corr:aspg_convergence}, we can still achieve an iteration complexity of $O(1/\epsilon^2)$ and  achieve a linear speedup when the number of workers is upper bounded by $O(K^{1/4}N^{-1/4})$. The major difference here is that, if we treat $M$ as a variable, the iteration complexity becomes $O(M/N\epsilon^2)$, which means that, the inconsistency among blocks does affect the iteration complexity. However, this does not imply the inefficiency of block-wise updates in Algorithm~\ref{alg:abpsgd-global}. This is due to the way we count iterations: in each iteration of Algorithm~\ref{alg:abpsgd-global}, a single block of $x$ instead of all $M$ blocks is updated. %If we take into account this fact when comparing to AsynSPG (Algorithm 1), the iteration complexity is essentially consistent. This comparison implies that the ``inconsistent read'' would not make a big difference from the ``consistent read''.

% \section{Discussion}
% \label{sec:discuss}

% Our results in Sec.~\ref{sec:aspg} and Sec.~\ref{sec:baspg} have shown that stochastic proximal gradient methods and stochastic gradient descent methods have the same convergence rate. In this section, we provide some further discussion and possible generalizations of our work. Due to space limit, we omit the details here.

% \testbf{Batch size}:
% Previous work for nonconvex nonsmooth optimization requires increasing batch size during training. Although our results show convergence with constant batch size, it is straitforward to obtain the convergence rate results when increasing batch size.

% \textbf{}
